Probabilistic Ensemble of Collaborative Filters

Collaborative filtering is an important technique for recommendation. Whereas it has been repeatedly shown to be effective in previous work, its performance remains unsatisfactory in many real-world applications, especially those where the items or users are highly diverse. In this paper, we explore an ensemble-based framework to enhance the capability of a recommender in handling diverse data. Specifically, we formulate a probabilistic model which integrates the items, the users, as well as the associations between them into a generative process. On top of this formulation, we further derive a progressive algorithm to construct an ensemble of collaborative filters. In each iteration, a new filter is derived from re-weighted entries and incorporated into the ensemble. It is noteworthy that while the algorithmic procedure of our algorithm is apparently similar to boosting, it is derived from an essentially different formulation and thus differs in several key technical aspects. We tested the proposed method on three large datasets, and observed substantial improvement over the state of the art, including L2Boost, an effective method based on boosting.

==> qualtab.tex <==

\begin{table*}
	\centering
	\caption{Examples in MovieLens Recommendation}
	\label{tab:MovieLensRec}
	\begin{tabular}{c|p{6cm}<{\centering}|p{6cm}<{\centering}|c}
		\hline
		& Movies & Genres & User Like? \\
		\hline
		\hline
		\multirow{10}{*}{Top 10 for User I} & Manhattan (1979) & Comedy$|$Drama$|$Romance & $\surd$ \\
		\cline{2-4}
		& Rebecca (1940) & Drama$|$Mystery$|$Romance$|$Thriller & $\surd$ \\
		\cline{2-4}
		& The Third Man (1949) & Film-Noir$|$Mystery$|$Thriller & $\surd$ \\
		\cline{2-4}
		& Vertigo (1958) & Drama$|$Mystery$|$Romance$|$Thriller & $\surd$ \\
		\cline{2-4}
		& Blue Velvet (1986) & Drama$|$Mystery$|$Thriller & $\surd$ \\
		\cline{2-4}
		& Hannah and Her Sisters (1986) & Comedy$|$Drama$|$Romance & $\surd$ \\
		\cline{2-4}
		& Chinatown (1974) & Crime$|$Film-Noir$|$Mystery$|$Thriller & $\surd$ \\
		\cline{2-4}
		& The Conversation (1974) & Drama$|$Mystery & $\surd$ \\
		\cline{2-4}
		& The Hours (2002) & Drama$|$Romance & $\surd$ \\
		\cline{2-4}
		& Before Sunset (2004) & Drama$|$Romance & $\surd$ \\
		\hline
		\hline
		\multirow{10}{*}{Top 10 for User II} & The Player (1992) & Comedy$|$Crime$|$Drama & $\surd$ \\
		\cline{2-4}
		& Raging Bull (1980) & Drama & $\surd$ \\
		\cline{2-4}
		& Touch of Evil (1958) & Crime$|$Film-Noir$|$Thriller & $\surd$ \\
		\cline{2-4}
		& Chinatown (1974) & Crime$|$Film-Noir$|$Mystery$|$Thriler & $\surd$ \\
		\cline{2-4}
		& Crumb (1994) & Documentary & $\surd$ \\
		\cline{2-4}
		& Raising Arizona (1987) & Comedy & $\surd$ \\
		\cline{2-4}
		& The Godfather (1972) & Crime$|$Drama & $\surd$ \\
		\cline{2-4}
		& The Wild Bunch (1969) & Adventure$|$Western & $\times$ \\
		\cline{2-4}
		& Pulp Fiction (1994) & Comedy$|$Crime$|$Drama$|$Thriller & $\surd$ \\
		\cline{2-4}
		& Do the Right Thing (1989) & Drama & $\times$ \\
		\hline
		\hline
		\multirow{10}{*}{Top 10 for User III} & Donnie Darko (2001) & Drama$|$Mystery$|$Sci-Fi$|$Thriller & $\surd$ \\
		\cline{2-4}
		& Eternal Sunshine of the Spotless Mind (2004) & Drama$|$Romance$|$Sci-Fi & $\surd$ \\
		\cline{2-4}
		& I Heart Huckabees (2004) & Comedy & $\surd$ \\
		\cline{2-4}
		& Amelie (2001) & Comedy$|$Romance & $\times$ \\
		\cline{2-4}
		& Pan's Labyrinth (2006) & Drama$|$Fantasy$|$Thriller & $\times$ \\
		\cline{2-4}
		& Spirited Away (2001) & Adventure$|$Animation$|$Fantasy & $\surd$ \\
		\cline{2-4}
		& Lost in Translation (2003) & Comedy$|$Drama$|$Romance & $\times$ \\
		\cline{2-4}
		& The Royal Tenenbaums (2001) & Comedy$|$Drama & $\times$ \\
		\cline{2-4}
		& Mulholland Drive (2001) & Crime$|$Drama$|$Film-Noir$|$Mystery$|$Thriller & $\times$ \\
		\cline{2-4}
		& Adaptation (2002) & Comedy$|$Drama$|$Romance & $\surd$ \\
		\hline
	\end{tabular}
\end{table*}

